Dense Air Quality Maps Using Regressive Facility Location Based Drive By Sensing

Currently, fixed static sensing is a primary way to monitor environmental data like air quality in cities. However, to obtain a dense spatial coverage, a large number of static monitors are required, thereby making it a costly option. Dense spatiotemporal coverage can be achieved using only a fraction of static sensors by deploying them on the moving vehicles, known as the drive by sensing paradigm. The redundancy present in the air quality data can be exploited by processing the sparsely sampled data to impute the remaining unobserved data points using the matrix completion techniques. However, the accuracy of imputation is dependent on the extent to which the moving sensors capture the inherent structure of the air quality matrix. Therefore, the challenge is to pick those set of paths (using vehicles) that perform representative sampling in space and time. Most works in the literature for vehicle subset selection focus on maximizing the spatiotemporal coverage by maximizing the number of samples for different locations and time stamps which is not an effective representative sampling strategy. We present regressive facility location-based drive by sensing, an efficient vehicle selection framework that incorporates the smoothness in neighboring locations and autoregressive time correlation while selecting the optimal set of vehicles for effective spatiotemporal sampling. We show that the proposed drive by sensing problem is submodular, thereby lending itself to a greedy algorithm but with performance guarantees. We evaluate our framework on selecting a subset from the fleet of public transport in Delhi, India. We illustrate that the proposed method samples the representative spatiotemporal data against the baseline methods, reducing the extrapolation error on the simulated air quality data. Our method, therefore, has the potential to provide cost effective dense air quality maps.

==> Intro_8sept.tex <==
\section{Introduction}
Air pollution has drawn attention in recent years because of its profound effect on people's health \cite{who:2019}. It is crucial to assess the pollution level in a region by monitoring the air quality levels and recommend strategies to combat pollution. There are significant factors that affect the air quality of an area, such as transportation, electricity, fuel uses, industrial parameters such as power plant emissions, etc. Hence, air quality monitoring is required to make strategies for emission control as well as verifying strategies that control emissions. \par

The most widely used method to monitor air quality is by using static sensing that is mounting sensors at fixed locations. The temporal resolution of static sensing is high, i.e., the air quality data is available for almost all the sampled timestamps. However, the spatial coverage in a region depends on the number of sensors installed which is generally limited owing to the cost constraints. As an illustration, a typical city in India requires in the order of thousand sensors to effectively capture a one square Km spatial resolution data.  An alternative and cost effective solution to provide a dense air quality map by using drive-by sensing, where static sensors are placed on mobile vehicles \cite{anjomshoaa2018city,hasenfratz2015deriving} and the monitoring is performed on the route traversed by the vehicle. Effectively, drive-by sensors can provide good coverage of the measurements across the region at the cost of not performing a high resolution temporal sensing like in static sensing. In other words, the moving sensors reading would be spatially and temporally sparse and incomplete because of the unavailability of the vehicle across all the spatial locations and timestamps. \par 

Thanks to the inherent temporal and spatial redundancy available in the air quality data, one can potentially impute the remaining (incomplete) data by utilising the matrix completion techniques \cite{asif2016matrix,ownwork} and obtain a dense air quality map in a fraction of the corresponding fixed sensing cost. The quality of imputation however crucially relies on the ``quality” of drive-by-sensing and the choice of ``routes” that vehicles take to sample the air quality. 
%PB Comment: above line can be expanded to explain why drive by sensing does not yield random sampling and therefore MC methods may not be that effective.
This paper addresses the problem of the choice of efficient drive-by-sensing routes for the city of Delhi. In our work, we investigate the usage of public transit buses for drive-by-sensing.  In a nutshell, we pick those routes that exploit the spatio-temporal structure in the air quality data resulting in an effective imputation and therefore achieving the required dense air quality map.

Researchers have worked on the choice of optimal static locations for fixed air quality sensing \cite{static1, static3,static2}, however not to our knowledge on mobile sensing.  The approach is to pick the subset of available static nodes and sample such that data on non selected subset of sites can be estimated with minimum error.  Selective drive by sensing, i.e., sampling the vehicle based on the routes, is different than the static sampling of sensors as distinct locations are sampled at different time stamps. Further, the literature on static node selection assumes that the ground truth data is available, and the sampling set can be picked based on minimizing the estimation error for the unsampled locations\cite{static1, static3}. However, it is unrealistic to assume the availability of the ground truth data before deploying the sensors, especially in the case of drive by sensing.  Therefore, sampling different sites using mount vehicles at different time stamps and the non-availability of the ground truth sensor readings differentiate our problem from the above mentioned works.\par

The problem of dense air quality maps using drive by sensing 
is defined as: Given a spatiotemporal matrix, where space refers to the locations, and temporal denotes the different time slots. Also, provided the occupancy data, the set of entries sampled in the spatiotemporal matrix for all the buses. The aim is to pick those sets of buses that perform representative sampling in the spatiotemporal matrix such that dense air quality maps can be obtained with minimum error. 
%PB Comment: above para has to be rewritten.

A naive way to choose the set of buses is to consider each entry in the spatiotemporal matrix as independent and try to maximize the number of entries in the matrix. However, this framework considers the entries in the matrix to be independent.

 Considering all the locations as independent ignores the correlation across locations, thereby highlighting the sub-optimality of such an approach. Indeed, sampling two consecutive neighborhood locations are less effective than sampling the diverse spread across locations in an area. In our work, we exploit the smoothness in the spatial locations to select buses that sample diverse and representative sets of locations. 

%PB Comment: above line should be reworded. Its not coming out well. 

Further, the air quality data for a given location is smooth in time, i.e., the sensor data varies slowly in time with decreasing correlation as the interval increases. Thereby, sampling the consecutive timestamps of a site is a less effective strategy than sampling at distant time stamps. 
We exploit the time series smoothness while sampling by assuming an autoregressive time series model on the spatio-temporal data.  Also, since the future temporal data is available to create the dense map at a particular timestamp, we use the causal temporal smoothness in the spatio-temporal data. This ensures that if a location $l$ is sampled at a given time, other buses can avoid sampling location $l$ and the nearby locations in the subsequent neighboring future time stamps. In other words, we exploit both location and temporal smoothness of the sensor signal in the proposed regressive facility location based drive by sensing framework. The regressive facility location (RFL) framework aims to encapsulate the slowly varying temporal data structure into the facility location framework and select the buses such that the sampled locations will be representative of the area and will be diverse across all time stamps.
 Practically it is not possible to access the real-world air quality data without deploying the sensors on the selected set of buses. Therefore, to evaluate the performance of the proposed regressive drive by sensing framework, we simulate real-world air quality data. Further, we obtain the dense air quality maps using the matrix completion framework using the sampled spatio-temporal data and observe that regressive facility locations provide more accurate dense air quality maps. 
 
	
	
	
	

The overall contribution of our work are:
\begin{enumerate}
\item We propose Regressive Facility Location (RFL), a novel method to select a fleet of vehicles(buses) for drive by sensing that incorporates the smoothness of the sensor reading across space as well as time to provide effective data sampling. 
\item We show that the proposed RFL algorithm gain is submodular, therefore a greedy heuristic provides a solution within an approximation ratio of  $(1-\frac{1}{e})$. 
\item We simulate the smooth data over space and time and sample the area using the proposed drive by sensing framework. To evaluate the performance of the proposed framework, we create dense maps using a matrix completion framework from the sampled data. 
\end{enumerate}


==> intro_old.tex <==

\section{Introduction}

Air quality has drawn attention in recent years because of its effect on people's health, causing cardiovascular diseases, lung cancer, etc. More than 90\% of the people are exposed to air quality levels that exceed the safe WHO guideline level for fine particulate matter (PM 2.5) \cite{who:2019}. It is crucial to assess the pollution level in a region to validate air quality standards.  The air quality of an area is impacted by multidimensional factors, including location and time. Therefore, it is necessary to sample the air quality of a region to monitor the air quality levels and recommend strategies to combat pollution. There are significant factors that affect the air quality of an area, such as transportation, electricity, fuel uses, industrial parameters such as power plant emissions, etc. Hence, air quality monitoring is required to make strategies for emission control, verifying those strategies for emission control, provide the air quality data to the general public so that they can make decisions regarding their health.\par




The most common scheme of monitoring air quality is using sensors at fixed locations and can be referred to as static sensing.  The temporal resolution of such sensing is high, i.e., the air quality data will be available for all the sampled timestamps. However, spatial coverage is limited and depends on the number of sensors to be installed. A higher percentage of sensors are required to provide the dense air quality map of an area, which is costly. A more efficient solution to provide a dense air quality map of the city to use drive-by sensing where sensors can be placed on mobile vehicles \cite{anjomshoaa2018city,hasenfratz2015deriving}. The air quality will be monitored on the route traversed by the vehicle. Thereby, drive-by sensors can improve coverage of the measurements across the region. However, the sensors reading would be spatially and temporally sparse because of the unavailability of the vehicle across all the spatial locations and timestamps. Moreover, the coverage across locations and time depends on the routes traversed by the vehicles. Therefore, it is crucial to pick the vehicles with the routes that provide the most effective coverage of an area. 


%There are two steps to create a dense air quality map for an area. The first is to sample the best representative sampling set of the city in space and time, and the second is the extrapolation or imputation of the data based on the sampled set. The second problem is discussed already in detail in various literature with the missing data imputation problem. However, there has been limited research on the sampling problem. 


Sampling for the static locations is discussed in the literature\cite{static1, static3,static2}. The approach is to pick the best subset of static nodes such that non selected subset of sites can be predicted with minimum error.  Selective drive by sensing, i.e., sampling the vehicle based on the routes, is different than the static sampling of sensors as distinct locations are sampled at different time stamps. Literature on selecting static nodes assumes that the ground truth data is available, and the sampling set can be picked based on minimizing the prediction error for the unsampled locations\cite{static1, static3}. However, it is unrealistic to assume that the ground truth data is already available before deploying the sensors, especially in the case of drive by sensing.  Therefore, sampling different sites using mount vehicles at different time stamps and the non-availability of the ground truth sensor readings differentiate our problem from the other sampling sensor-based algorithms.\par

There are mainly two ways of drive by sensing, either we can pick the best routes for sampling and run dedicated vehicles on those routes or pick the vehicles with fixed routes. However, dedicating vehicle for sampling is an expensive idea. Therefore, a more affordable solution is Public transportation, i.e., buses that operate on fixed routes can be used for drive by sensing. Thereby, we explore the problem of selecting the best set of buses that can be used for drive by sensing to obtain a dense air quality map for the entire city. 



% Also, provided improve
The problem of dense air quality maps using drive by sensing 
is defined as: Given a spatiotemporal matrix, where space refers to the locations, and temporal denotes the different time slots. Also, provided the occupancy data, the set of entries sampled in the spatiotemporal matrix for all the buses. The aim is to pick those sets of buses that perform representative sampling in the spatiotemporal matrix such that dense air quality maps can be obtained with minimum error. 


The naive way to choose the set of buses is to consider each entry in the spatiotemporal matrix as independent and try to maximize the number of entries in the matrix, which in turn improves the sampling percentage in the matrix. However, this framework considers the entries in the matrix to be independent \cite{related1, related4}.  
%One such methods proposed for drive by sensing is to maximize the percentage coverage in the sampling matrix $\X(\M)= \max\limits_{l \in \L, t \in \T}(\sum\limits_{ k \in \M} \Y_{l,t,k},1)$ where $\M$ is the selected set of buses from $\B$ \cite{agarwal2020modulo}. 


%Since the sensor readings are smooth in space and time, the air quality measurements vary slowly in space and time; therefore, the signal is band-limited in space and time. So uniform samples across space and time can be a potential way to sample the data, and most of the imputation-based strategies involve the measurements to be uniformly missing. However, uniform sampling is not possible in the case of drive-by sensing as the vehicles follow a pattern. \par


Considering all the locations as independent does not account for the diversity of the entire space. Sampling two consecutive neighborhood locations are less effective than sampling the diverse spread across locations in an area. 
We thereby exploit the smoothness in the spatial locations to select buses that sample diverse and representative sets of locations. Furthermore, the sensor data is smooth in time, i.e., the sensor data varies slowly in time. Thereby, sampling the consecutive timestamps of a site is a less effective strategy than sampling at distant time stamps. We exploit the time series smoothness while sampling by assuming an autoregressive time series model on the spatiotemporal data. Also, since the future temporal data is not available to create the dense map at a particular timestamp, we use the causal temporal smoothness in the spatiotemporal data. This ensures that if a location $l$ is sampled at a given time, other buses can avoid sampling location $l$ and the nearby locations in the subsequent future time stamps. Thereby, we exploit both location and temporal smoothness of the sensor signal in the proposed regressive facility location based drive by sensing framework. 

 Practically it's not possible to access the real-world air quality data without deploying the sensors on the selected set of buses. Therefore, to evaluate the performance of the proposed regressive drive by sensing framework, we simulate the real-world air quality data. Further, we obtain the dense air quality maps using the matrix completion framework using the sampled spatiotemporal data and observe that regressive facility locations provide more accurate dense air quality maps. 
 
 

% Treating the locations as independent would not differentiate if the $m$ sites that are sampled are in the neighborhood or diversely spread across the area. However, if we are sampling $m$ sites, we want the sampled sites to be diverse and representative of the entire area. Sensor data varies slowly over the neighboring regions; therefore, there is a smoothness in the spatial locations. Thereby, we can exploit the smoothness in the spatial locations to select the buses. 
%, which in turn samples the sites representing the entire location space. 
%We can use a Facility location-based framework for all the timestamps. 


The overall contribution of our work are:
\begin{enumerate}
%	\item We propose Regressive Facility Location (RFL), a novel method to select the vehicles for drive by sensing that provides the samples which are representative of the entire area while incorporating the autoregressive time structure in the sampling. 
\item We propose Regressive Facility Location (RFL), a novel method to select a fleet of vehicles (buses) for drive by sensing that incorporates the smoothness of the sensor reading across space as well as time to provide effective data sampling. 
\item We showed that the proposed RFL algorithm gain is submodular, therefore a greedy heuristic provides a solution within an approximation ratio of  $(1-\frac{1}{e})$. 
\item We stimulate the smooth data over space and time and sample the area using the proposed drive by sensing framework. To evaluate the performance of the proposed framework, we create dense maps using a matrix completion framework from the sampled data. 

\end{enumerate}

%	Smoothly varying signals defined on the nodes are of particular interest in various applications, and tend to be approximately bandlimited in the frequency basis. 

%	The overall contribution of our work are: We present a selective drive by sensing an efficient sampling framework that incorporates the smoothness of the sensor reading across space as well as time to provide effective data sampling. 


